Dynamic Swarm Dispersion in Particle Swarm Optimization for Mining Unsearched Area in Solution Space (DSDPSO)

Premature convergence in particle swarm optimization (PSO) algorithm usually leads to gaining local optimum and preventing from surveying those regions of solution space which have optimal points in. In this paper, by applying special mechanisms, suitable regions were detected and then swarm was guided to them by dispersing part of particles on proper times. This process is called dynamic swarm dispersion in PSO (DSDPSO) algorithm. In order to specify the proper times and to rein the evolutionary process alternating between exploring and exploiting behaviors, we used a diversity measuring approach and implemented the dispersion mechanism. To promote the performance of DSDPSO algorithm, three different policies including particle relocation, velocity settings of dispersed particles and parameters setting were applied. We compared the promoted algorithm with similar new approaches and according to the numerical results, the proposed algorithm outperformed the basic GPSO, LPSO, DMS-PSO, CLPSO and APSO in most of the 12 standard benchmark problems with different properties taken in this study.

==> DSDPSO.bbl.tex <==
\begin{thebibliography}{}

\bibitem[Bahrampour and Mohamad Nezami, 2013]{1}
Bahrampour, A. and O. Mohamad Nezami (2013).
\newblock Diversity guided particle swarm optimization (DGPSO) algorithm based on search space awareness particle dispersion.
\newblock {\em Proceedings of the 15th International Conference on Artificial Intelligence (ICAI 2013)}.
\newblock Volume 2,
\newblock pp. 218-224.
\newblock Las Vegas Nevada,
\newblock USA.

\bibitem[Blackwell and Bentley, 2002]{2}
Blackwell, T. M. and P. Bentley (2002).
\newblock Don’t push me! Collision-avoiding swarms.
\newblock {\em Proceedings of the IEEE Congress on Evolutionary Computation (CEC 2002)}.
\newblock Volume 2,
\newblock pp. 1691-1696.
\newblock Honolulu,
\newblock USA.

\bibitem[Chang et al., 2010]{3}
Chang, P. C., W. H. Huang, and C. J. Ting (2010).
\newblock Dynamic diversity control in genetic algorithm for mining unsearched solution space in TSP problems.
\newblock {\em Expert Systems with Applications 37(3)},
\newblock 1863-1878. 

\bibitem[Cheng and Shi, 2011]{4}
Cheng, S. and Y. Shi (2011).
\newblock Diversity control in particle swarm optimization.
\newblock {\em Proceedings of the IEEE Symposium on Swarm Intelligence (SIS 2011)}.
\newblock pp. 1-9.
\newblock Paris,
\newblock France.

\bibitem[Dong et al., 2008]{5}
Dong, D., J. Jie, J. Zeng, and M. Wang (2008).
\newblock Chaos-mutation-based particle swarm optimizer for dynamic environment.
\newblock {\em Proceedings of the 3rd International Conference on Intelligent System and Knowledge Engineering (ISKE 2008)}.
\newblock Volume 1,
\newblock pp. 1032-1037.
\newblock Xiamen,
\newblock China.

\bibitem[Eberhart et al., 1996]{6}
Eberhart, R., R. Dobbins, and P. Simpson (1996).
\newblock {\em Computational Intelligence PC Tools}.
\newblock Academic Press Professional.

\bibitem[Eberhart and Kennedy, 1995a]{7}
Eberhart, R. and J. Kennedy (1995a).
\newblock A new optimizer using particle swarm theory.
\newblock {\em Proceedings of the 6th International Symposium on Micro Machine and Human Science}.
\newblock  pp. 39-43.
\newblock Nagoya,
\newblock Japon.

\bibitem[Higashi and Iba, 2003]{8}
Higashi, N. and H. Iba (2003).
\newblock Particle swarm optimization with Gaussian mutation.
\newblock {\em Proceedings of the IEEE Swarm Intelligence Symposium}. 
\newblock pp. 72-79.
\newblock Indianapolis,
\newblock USA.

\bibitem[Jie et al., 2006]{9}
Jie, J., J. Zeng, and  C. Han (2006).
\newblock Adaptive particle swarm optimization with feedback control of diversity.
\newblock {\em Proceedings of the International Conference on Intelligent Computing (ICIC 2006)}. 
\newblock pp. 81–92.
\newblock Kunming, 
\newblock China.

\bibitem[Kennedy and Eberhart, 1995b]{10}
Kennedy, J. and  R. Eberhart (1995b).
\newblock Particle swarm optimization.
\newblock {\em Proceedings of the IEEE International Conference on Neural Networks (ICNN 1995)}.
\newblock Volume 4,
\newblock pp. 1942-1948.
\newblock Perth,
\newblock Australia.

\bibitem[Krohling, 2005]{11}
Krohling, R. A.(2005).
\newblock Gaussian particle swarm with jumps.
\newblock {\em Proceedings of the IEEE Congress on Evolutionary Computation}.
\newblock pp. 1226-1231.
\newblock Edinburg,
\newblock Scotland.

\bibitem[Li and Engelbrecht, 2007]{12}
Li, X. and  A. P. Engelbrecht (2007).
\newblock Particle swarm optimization: An introduction and its recent developments.
\newblock {\em Proceedings of the Genetic and Evolutionary Computation Conference (GECCO 2007)}.
\newblock pp. 3391-3414.
\newblock London, 
\newblock UK.

\bibitem[Liang and Suganthan, 2005]{13}
Liang, J. J. and  P. N. Suganthan (2005).
\newblock Dynamic multi-swarm particle swarm optimizer with local search.
\newblock {\em Proceedings of the IEEE Congress on Evolutionary Computation}.
\newblock Volume 1,
\newblock pp. 522–528.
\newblock Edinburgh, 
\newblock Scotland.

\bibitem[Liang et al., 2006]{14}
Liang, J. J., A. K. Qin, P. N. Suganthan, and S. Baskar (2006).
\newblock Comprehensive learning particle swarm optimizer for global optimization of multimodal functions.
\newblock  {\em IEEE Transactions on Evolutionary Computation 10(3)}, 
\newblock 281-295.

\bibitem[Lovbjerg and Krink, 2002]{15}
Lovbjerg, M. and T. Krink (2002).
\newblock Extending particle swarm optimisers with self-organized criticality.
\newblock {\em Proceedings of the IEEE Congress on Evolutionary Computation (CEC 2002}.
\newblock Volume 2,
\newblock pp. 1588-1593.
\newblock Honolulu,
\newblock USA.

\bibitem[Mohamad Nezami and Bahrampour, 2013]{16}
Mohamad Nezami, O. and  A. Bahrampour (2013).
\newblock Particle swarm optimization algorithm based on diversified artificial particles (PSO-DAP).
\newblock {\em Proceedings of the 11th Iranian Conference on Intelligent Systems}.
\newblock Tehran,
\newblock  Iran.

\bibitem[Mohamad Nezami et al., 2013]{17}
Mohamad Nezami, O., A. Bahrampour, and P. Jamshidlou (2013).
\newblock Dynamic diversity enhancement in particle swarm optimization (DDEPSO) algorithm for preventing from premature convergence.
\newblock {\em Proceedings of the 17th Asia Pacific Symposium on Intelligent and Evolutionary Systems (IES)}.
\newblock Seoul, 
\newblock South Korea.

\bibitem[Parsopoulos and Vrahatis, 2004]{18}
Parsopoulos, K. E. and M. N. Vrahatis (2004).
\newblock On the computation of all global minimizers thorough particle swarm optimization.
\newblock {\em IEEE Transactions on Evolutionary Computation 8(3)},
\newblock 211-224.

\bibitem[Riget and Vesterstrorm, 2002]{19}
Riget, J. and J. S. Vesterstrorm (2002).
\newblock A Diversity guided particle swarm optimizer–The ARPSO.
\newblock {\em Technical Report}.
\newblock Department of Computer Science,
\newblock University of Aarhus,
\newblock Denmark.

\bibitem[Secrest and Lamont, 2003]{20}
Secrest, B. R. and G. B. Lamont (2003).
\newblock Visualizing particle swarm optimization–Gaussian particle swarm optimization.
\newblock {\em Proceedings of the IEEE Swarm Intelligence Symposium (SIS 2003)}.
\newblock pp. 198-204. 
\newblock Indianapolis, 
\newblock USA.

\bibitem[Shi and Eberhart, 2009]{21}
Shi, Y. and  R. Eberhart (2009).
\newblock Monitoring of particle swarm optimization.
\newblock {\em Frontiers of Computer Science in China 3(1)},
\newblock 31-37.
\newblock SP Higher Education Press.

\bibitem[Shi and Eberhart, 2008]{22}
Shi, Y. and R. Eberhart (2008).
\newblock Population diversity of particle swarms.
\newblock {\em Proceedings of the IEEE Congress on Evolutionary Computation (CEC 2008)}.
\newblock pp. 1063-1067.
\newblock Hong Kong.

\bibitem[Soleymani et al., 2007]{31}
Soleymani, S., A. M. Ranjbar, S. Bagheri Shoukari, A. R. Shirani, and N. Sadati (2007).
\newblock A new approach for bidding strategy of gencos using  
particle swarm optimization combined with simulated annealing method.
\newblock {\em Iranian Journal of Science \& Technology, Transaction B, Engineering}. 
\newblock Volume 31, 
\newblock No. B3,  
\newblock pp. 303-315.
\newblock Shiraz University,
\newblock Iran.

\bibitem[Sriyanyong, 2008]{23}
Sriyanyong, P.(2008).
\newblock Solving economic dispatch using Particle Swarm Optimization combined with Gaussian mutation.
\newblock {\em Proceedings of the 5th International Conference on Electrical Engineering/Electronics, Computer, Telecommunications and Information Technology (ECTI-CON 2008)}. 
\newblock Volume 2,
\newblock pp. 885-888. 
\newblock Krabi,
\newblock Thailand.

\bibitem[Stacey et al., 2003]{24}
Stacey, A., M. Jancic, and I. Grundy (2003).
\newblock Particle swarm optimization with mutation.
\newblock {\em Proceedings of the IEEE Congress on Evolutionary Computation (CEC 2003)}.
\newblock Volume 2,
\newblock pp. 1425-1430.
\newblock Canberra,
\newblock Australia.

\bibitem[Wei et al., 2002]{25}
Wei, C., Z. He, Y. Zhang, and W. Pei (2002).
\newblock Swarm directions embedded in fast evolutionary programming.
\newblock {\em Proceedings of the IEEE Congress on Evolutionary Computation (CEC 2002)}. 
\newblock Volume 2,
\newblock pp. 1278-1283.
\newblock Honolulu,
\newblock USA.

\bibitem[Yang et al., 2009]{26}
Yang, M., H. Huang, and G. Xiao (2009).
\newblock A novel dynamic particle swarm optimization algorithm based on chaotic mutation.
\newblock {\em Proceedings of the 2nd International Workshop on Knowledge Discovery and Data Mining (KDD 2009)}. 
\newblock pp. 656-659.
\newblock Moscow,
\newblock Russia.

\bibitem[Yao et al., 1999]{27}
Yao, X., Y. Liu, and G. Lin (1999).
\newblock Evolutionary programming made faster.
\newblock {\em IEEE Transactions on Evolutionary Computation 3(2)}, 
\newblock 82-102.

\bibitem[Yue-Lin et al., 2008]{28}
Yue-Lin, G., A. Xiao-hui, and L. Jun-min (2008).
\newblock A particle swarm optimization algorithm with logarithm decreasing inertia weight and chaos mutation.
\newblock {\em Proceedings of the Conference on Computational Intelligence and Security (CIS 2008)}. 
\newblock Volume 1,
\newblock pp. 61-65.
\newblock Suzhou,
\newblock China.

\bibitem[Zhan et al., 2009]{29}
Zhan, Z. H.,  J. Zhang, Y. Li, and H. S. Chung (2009).
\newblock Adaptive particle swarm optimization.
\newblock {\em IEEE Transactions on Systems, Man, and Cybernetics, Part B: Cybernetics 39(6)}, 
\newblock 1362-1381.

\bibitem[Zhan et al., 2010]{30}
Zhan, Z., J. Zhang, and Y. Shi (2010).
\newblock Experimental study on PSO diversity.
\newblock {\em Proceedings of the 3rd International Workshop on Advanced Computational Intelligence (IWACI 2010)}. 
\newblock pp. 310-317.
\newblock Suzhou,
\newblock China.

\end{thebibliography}
